MASKDROID: Robust Android Malware Detection with Masked Graph Representations

Android malware attacks have posed a severe threat to mobile users, necessitating a significant demand for the automated detection system. Among the various tools employed in malware detection, graph representations (e.g., function call graphs) have played a pivotal role in characterizing the behaviors of Android apps. However, though achieving impressive performance in malware detection, current state-of-the-art graph-based malware detectors are vulnerable to adversarial examples. These adversarial examples are meticulously crafted by introducing specific perturbations to normal malicious inputs. To defend against adversarial attacks, existing defensive mechanisms are typically supplementary additions to detectors and exhibit significant limitations, often relying on prior knowledge of adversarial examples and failing to defend against unseen types of attacks effectively. In this paper, we propose MASKDROID, a powerful detector with a strong discriminative ability to identify malware and remarkable robustness against adversarial attacks. Specifically, we introduce a masking mechanism into the Graph Neural Network (GNN) based framework, forcing MASKDROID to recover the whole input graph using a small portion (e.g., 20%) of randomly selected nodes.This strategy enables the model to understand the malicious semantics and learn more stable representations, enhancing its robustness against adversarial attacks. While capturing stable malicious semantics in the form of dependencies inside the graph structures, we further employ a contrastive module to encourage MASKDROID to learn more compact representations for both the benign and malicious classes to boost its discriminative power in detecting malware from benign apps and adversarial examples.

==> backup/0_abstract.tex <==
Android malware attacks have posed a severe threat to mobile users, \za{necessitating a significant demand for the automated detection system.}
% Android malware attacks have posed a severe threat to mobile users. 
% Hence, there also arises a significant demand for the automated detection of Android malware.
% Given its important role in indicating the behavior of Android applications, Function Call Graph (FCG) has been widely adopted in Malware Detection. 
\za{Among the various tools employed in malware detection, Function Call Graphs (FCGs) have played a pivotal role by characterizing the behavior of Android applications.} 
However, though achieving impressive \za{performance} in malware detection, current state-of-the-art FCG-based detectors are \za{vulnerable} to adversarial examples.
% crafted by adding carefully chosen perturbations to the normal malicious inputs. 
\za{These adversarial examples are meticulously crafted by introducing specific perturbations to normal malicious inputs.
To defend against adversarial attacks, existing defensive mechanisms are typically supplementary additions to detectors and exhibit significant limitations, often relying on prior knowledge of adversarial examples and failing to effectively defend against unseen types of attacks. }
% researchers have mainly focused on two categories of approaches: data perspective and model perspective. 
% Unfortunately, the usability and effectiveness of these defensive mechanisms are significantly limited since they usually require knowledge of adversarial examples and cannot defend against unseen types of attacks. 

In this paper, we \za{propose} \codename, a detector model that not only possesses strong \za{discriminative} power to identify malware but also demonstrates robustness against adversarial
attacks. 
Specifically, we introduce a random masking technique into the Graph Neural Network (GNN) based framework, forcing \za{ \codename  recover the whole FCG} using a small portion of (\textit{e.g.}, 20\%) randomly selected nodes. 
This strategy largely reduces redundancy and compels the \za{detector} to understand the malicious structures within FCGs holistically beyond low-level trivial statistics. 
\za{By} capturing stable malicious structures in the form of dependencies inside FCGs, \codename is able to stand robust against non-malicious structural changes designed by adversaries. 
Additionally, we employ a proxy-based contrastive loss to further enhance the \za{detector's} discriminative power. 
Extensive experiments validate the effectiveness \za{of  \codename } to detect malware in real-world scenarios comparable to SOTA approaches while showcasing advanced robustness against \za{various} adversarial attacks. 
\za{Our codes are available at \url{https://anonymous.4open.science/}.}

==> backup/1_introduction.tex <==

\section{Introduction}

% Android stands as one of the most popular smartphone operating systems (OSs) dominating more than 85\% of the mobile OS market share since 2018 \cite{li2018significant}. 
% Unfortunately, due to its openness and popularity, Android has also become one of the primary targets of cyberattacks \cite{liu2022deep}. 
\za{Android, as one of the most prevalent smartphone operating systems,} has dominated over 85\% of the mobile OS market share since 2018~\cite{li2018significant}.
However, its popularity and open nature have also made it a primary target for cyberattacks~\cite{liu2022deep, judy}.
\za{Vulnerabilities in open-source components can be easily exploited in the Andriod applications integrating them.}
%In contrast to other platforms, Android permits the installation of applications from unverified sources, such as third-party markets, thereby providing attackers with easy means to bundle and distribute malware-infected apps \cite{arp2014drebin}.
% Symantec reported that one in every five Android applications is actually malware, a.k.a., malicious application \cite{symantec2019internet}.
% For instance, in 2017, the Judy malware infected approximately 36 million Android devices, causing serious economic losses via fraudulent activities~\cite{judy}.
% Since attackers can exploit these malware to compromise user privacy or execute perilous operations on their devices, they are posing a severe threat to mobile users.
% Since Function call graph (FCG) provides important clues for understanding the behaviors of Android applications (app for short), it has been widely adopted in Android Malware Detection (AMD) \cite{mamadroid, wu2019malscan, wu2021homdroid, hou2017hindroid, he2022msdroid}. 
% In particular, FCG encapsulates the caller-callee relationships among the API calls in an app, where nodes represent the api calls, and edges denote method invocation\cite{li2023black}.
\za{In response to the increasing number of vulnerability disclosures, developers increasingly value function call graphs (FCGs) for comprehensive vulnerability assessments before app installation~\cite{mamadroid, wu2019malscan, he2022msdroid}.}
%In response to such threats, the Function Call Graph (FCG) has been widely used to detect Android malware before app installation~\cite{mamadroid,wu2019malscan,he2022msdroid}.
%This is because FCG encapsulates the caller-callee relationship among the API calls in an app, offering invaluable insights into the behavioral patterns of APKs~\cite{li2023black}.
\za{FCGs encapsulate the caller-callee relationship among API calls in an app, facilitating an understanding of whether and how a vulnerability can be invoked—a pivotal factor for being exploitable and susceptible to attacks.}
\za{Consequently, FCGs have gained widespread adoption in Android malware detection, offering invaluable insights into the behavioral patterns of Android Application Packages (APKs)~\cite{li2023black}.}

%In an FCG, every node represents a function in the Java source code of the application, and every edge denotes the calling relationship between caller and callee.

\za{While current state-of-the-art FCG-based detectors have demonstrated impressive performance in malware detection, these neural network-based models are susceptible to adversarial examples (AEs) crafted by carefully introducing perturbations to malicious inputs~\cite{chen2019android, zhao2021structural, zhang2022semantics}.} 
% Though achieving impressive \za{performance} in malware detection, current state-of-the-art FCG-based detectors are susceptible to adversarial examples (AEs)~\cite{chen2019android, zhao2021structural, zhang2022semantics}, crafted by adding carefully chosen perturbations to the malicious inputs.
% \jiahao{this part discusses neural networks directly, there is a gap}
%TODO: 这一句是否可以去掉？
This lack of robustness against adversarial attacks stems from the \za{well-known} nature of neural networks, \za{where} small but intentionally \za{designed perturbations can lead to incorrect predictions}
%result in an incorrect prediction result 
with high confidence~\cite{goodfellow2014, croce2020reliable, madry2017towards, athalye2018obfuscated}.
In the case of FCG data, adversarial examples are \za{specifically} generated by \za{targeting} the most influential edges/nodes for modification, \za{enabling malware inputs to evade the decision boundary and thereby undermining the detectors' performance} 
% to help the malware inputs evade the decision boundary, thus undermining the performance of the detectors
~\cite{wu2019adversarial, chen2019android, zhang2022semantics}.


% Rearrange this paragraph.
\za{Existing defensive mechanisms against adversarial attacks are typically supplementary additions to detector models, which inevitably require significant overhead during the implementation and further limit their applicability.
These additional defensive approaches can be broadly categorized into two groups: data perspective defenses~\cite{goodfellow2014, al2018adversarial, wang2017adversary} and model perspective defenses~\cite{distillation, grosse2016, li2020adversarial, chen2017securedroid}. 
Defenses from the data perspective suffer from a significant demand for labeled adversarial data and showcase limited effectiveness against unseen types of adversarial examples \cite{gu2014towards, ororbia2016unifying}.
Model perspective defenses, exemplified by defensive distillation, also achieve limited success due to the transferability of adversarial examples \cite{distillation}. 
Consequently, we contend that the current two groups of defensive mechanisms fall short of meeting the demands posed by adversarial attacks.
The truly ideal malware detector should not rely on external defense mechanisms but should inherently possess both a strong malware identification capability and robustness against \jz{adversarial} attacks.}
% To defend against adversarial attacks, researchers have mainly focused on two categories of approaches: data perspective \cite{goodfellow2014, al2018adversarial, wang2017adversary} and model perspective \cite{distillation, grosse2016, li2020adversarial, chen2017securedroid}. 
% Defenses from the data perspective suffer from a significant demand for labeled adversarial data and showcase limited success when faced with unseen types of adversarial examples \cite{gu2014towards, ororbia2016unifying}.
% Model perspective defenses, with defensive distillation being a prime example, also achieve limited success due to the transferability of adversarial examples \cite{distillation}. 
% Besides, since these defensive mechanisms are supplemental additions to detector models that require significant overhead during the implementation, their effectiveness is substantially limited. 
% In conclusion, existing defensive mechanisms fall short of meeting the demands posed by adversarial attacks.

% In this paper, to bridge the gap, we propose an ideal malware detector that not only possesses strong discrimination power to identify malware but also exhibits robustness against adversarial attacks. 
% In this paper, to bridge the gap, we propose \za{a powerful} malware detector, named \codename, that not only possesses strong \za{discriminative} power to identify malware but also exhibits robustness against adversarial attacks \za{without the need of employing extra defensive mechanisms}.
% We present a novel malware detection system called \codename with enhanced robustness before the employment of extra defensive mechanisms. 
\za{To bridge the gap,} understanding adversaries is the first step \za{towards} defeating them. 
Malware developers often conceal their intentions by mimicking the behavior of benign apps, embedding a small portion of malicious code (\textit{e.g.}, less than 2\%) within a bulk of benign processes \cite{medium, hou2017hindroid}. 
\za{When represented in the form of} an FCG, a malicious input is characterized as a small subgraph embedded within the overall call graph.  
Adversarial examples preserve the malicious code \za{responsible for} the behavior subgraph while strategically introducing additional nodes or edges to \za{confound} the detectors \cite{li2021robust}. 
Therefore, to establish a robust \za{defense} against malware and adversarial examples, a \za{detector} must \za{possess a comprehensive understanding of any subgraph within the FCG, \ie potential malicious structure.} 
% comprehensively understand the malicious structure to detect an input sample containing malicious behaviors without evasion, regardless of its camouflage.
\za{This understanding further enables the detector to identify input samples containing malicious behaviors, regardless of their camouflage.}

To force the \za{detector} to concentrate on the understanding of malicious behaviors inside FCG, we introduce a random \za{masking technique} into the Graph Neural Network (GNN) based framework. Specifically, during the training phase, we randomly mask out a substantial proportion (e.g., 80\%) of nodes in the input FCG, forcing \za{the detector to recover the removed representations using the remaining 20\% nodes.} 
%20\% of randomly selected nodes to recover the removed representations. 
\za{By doing so}, the \za{detector} is encouraged to capture the local patterns and dependencies \za{to reconstruct the masked-out portions effectively}. 
Therefore, this strategy forces the \za{detector} to \za{gain a holistic understanding of malicious structures, transcending mere statistical patterns~\cite{he2022masked, vincent2008extracting}.}
% understand the malicious structures holistically beyond trivial statistics \cite{he2022masked, vincent2008extracting}. 
While capturing the stable malicious structures in the form of dependencies inside FCGs, the \za{detector} is able to stand robust against non-malicious structural changes designed by adversaries.

With representations that comprehensively grasp the malicious structures, we proceed to apply binary classification \za{for detection.}
%Instead of using the traditional MLP, 
\za{To achieve this,} we leverage the proxy-based contrastive learning method as the binary detector, \za{which} enhances the detection of instances \za{containing} malicious structures, including both original malware and adversarial examples \cite{yao2022pcl}.
%\indent Additionally, we take advantage from the power of proxy-based contrastive learning to further enhance the discrimination power of the model \cite{yao2022pcl}.
\za{In this approach,} we initialize two proxy representations, \za{serving as anchors for} benign and malware classes, respectively. 
We optimize the proxy-to-sample relations to pull samples in the same class closer and push apart samples in different classes.
\za{Simultaneously, we update} the proxy representations to maintain their role as anchors \za{for the respective classes.}
Prediction is made by determining which proxy the instance is closer to. 
The contrastive loss encourages the detector to \za{encode} more compact representations for the inputs, thus enhancing \za{its ability} to detect both malware and adversarial examples. 

Overall speaking, \za{in this paper, we introduce \codename, a robust malware detector that not only excels in identifying malware with strong discriminative power but also exhibits robustness against adversarial attacks, eliminating the need for additional defensive mechanisms.}
\za{Specifically,} \codename is \za{founded on a GNN-based framework, which integrates a random masking technique for a deeper understanding of malicious structures and utilizes a proxy-based contrastive loss to boost its discriminative power for detecting.} 
% \codename is a GNN-based malware detector that incorporates a random mask to understand the malicious structures and a proxy-based contrastive loss to boost its discrimination power to detect them. 
We validate the effectiveness of \codename in real-world scenarios \za{through classification tasks and subject it to various} adversarial attacks, \za{highlighting its superior robustness compared to state-of-the-art malware detectors.}
%to prove its advanced robustness compared to SOTA malware detectors. 

The major contributions of this work include:


\begin{itemize}[leftmargin=12pt]
    \item 
    % To the best of our knowledge, this is the first attempt to enhance the robustness of the FCG-based malware detection model by addressing the model itself instead of applying a supplemental defensive strategy.
    To the best of our knowledge, this is the first attempt to enhance the robustness of the FCG-based malware detection model \za{against adversarial attacks} instead of applying a supplemental defensive mechanism.
    \item We present \codename, a novel GNN-based Android malware detector. It incorporates a random \za{masking technique} to \za{distill} malicious information within input instances and utilizes a proxy-based contrastive loss to \za{further} boost its ability \za{for detection}.
    \item  We conduct extensive experiments demonstrating that \codename possesses comparable effectiveness in the malware detection task compared to SOTA graph-based approaches.
    \za{Moreover, it achieves significantly superior robustness against adversarial attacks, marking a substantial improvement in malware detection.}
    % while achieving significantly better robustness against adversarial attacks.
\end{itemize}


==> backup/2_preliminary.tex <==
\section{Preliminary}
\section{Preliminary} \label{sec:prelimimary}
%\jiahao{The flow is okay --- easy to understand there are something can be improved.}
\indent We begin with the explanation of the graph-based Android Malware Detection. We first introduce the
graph representation of Android applications, and explain how are they are employed in malware detection. Then, we formulate the problem of  effectiveness and robustness in graph-based malware detection, and reveal the limitations of current SOTA detectors in achieving these goals. 
%Throughout the paper, we represent the random variables and their deterministic values with the upper-cased (\textit{e.g.}, $X$) and lower-cased (\textit{e.g.}, $x$) letters, respectively.


\subsection{Graph-based Android malware detection}
Android applications are packaged and distributed in the form of Android Package Kit (APK) files \cite{chen2019android}. 
%Given an APK, the objective of Android malware detection is to distinguish malicious apps from benign ones. Currently, researchers resolve this task by extracting program features from APK and train a machine learning (ML) based detection model. Features adopted in the existing literatures fall into two categories: dynamic and static \cite{chen2019android, tam2017evolution, fu2017leaksemantic, yuan2019lightweight, arp2014drebin, mamadroid, wu2019malscan}. Dynamic features, including network traffic, battery usage and IP addresses, are extracted by monitoring the behavior of apps at run-time, resulting in significant overhead \cite{yuan2019lightweight}. Therefore, static features obtained before the execution of apps are more common in practical applications \cite{li2021robust}.
Serving as an important indicator of APK behavior, Function Call Graph (FCG) has been widely adopted in Android Malware Detection (AMD)~\cite{mamadroid,wu2019malscan,he2022msdroid}. In particular, FCG encapsulates the caller-callee relationships among the API calls in an app, where nodes represent the api calls, and edges denote method invocation\cite{li2023black}. Researchers then perform representation learning on the 
constructed FCGs\cite{mamadroid, wu2019malscan, he2022msdroid}. 
Mamadroid \cite{mamadroid} abstracts the nodes of FCGs to their packages or families, before analyzing the sequence of abstracted function calls. Malscan \cite{wu2019malscan} performs centrality analysis to sensitive nodes in FCGs to represent the semantic features of the applications. MsDroid \cite{he2022msdroid} generates graph snippets around sensitive APIs and classify them by Graph Neural Network (GNN).

\subsection{Problem Formulation}
%\jiahao{I think we can introduce the FCG-based malware detection directly. For example, FCG-based Android malware detectors take FCG as input, and output the probability of the APK is malicious. Here, we formally define ...}\\
\noindent \textbf{Malware Detection.}   
%Android malware detection based on machine learning methods, can be described as a binary classification problem in which program features are extracted to train a detection model. The features we adopted here is the Function Call Graph (FCG), as it serves as an important indicator to capture the behavior and functionality of apps. 
FCG-based Android malware detectors take FCG as input, and output the probability of the APK is malicious. Here, we formally define the call graph as $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{X}) $, where each element $v \in \mathcal{V} $ represents an API and each edge $(e_1, e_2) \in \mathcal{E} $ indicates an invocation from $v_1$ to $v_2$ in the smali code. $\mathcal{X}$ represents the features of the nodes. 
An Android app is malicious as long as there exists malicious behavior, carried out by some malicious code. These malicious code are small snippets embedded within a bulk of benign code, with a proportion estimated at 0.18\% \cite{sikorski2012practical}. 
In that case, when represented with a call graph $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{X}) $,  a malware sample contains a collection of subgraphs \( \mathcal{H} = \{  \mathcal{H}_i = (\mathcal{V}_i, \mathcal{E}_i), \mathcal{X}  |  \mathcal{V}_i \subseteq \mathcal{V},   \mathcal{E}_i \subseteq \mathcal{E},  \mathcal{X}_i \subseteq \mathcal{X} \} \) such that each subgraph \(\mathcal{H}_i\) represents a snippet of malicious code. The task of a malware detector is to train a classifier  $\mathcal{C}: \mathcal{G} \rightarrow \{0, 1\}$ where 0 denotes a benign app, 1 denotes a malware. \\

%We propose that the goal of an ideal classifier is to achieve both effectiveness and robustness, defined as follows. 
\noindent \textbf{Adversarial Examples.} Adversarial examples are generated from malware instances with the intention of misleading the classifier while still preserving their malicious functionalities. In the case of a call graph, an adversarial examples can be represented as $\hat{\mathcal{G}} = \mathcal{G} + \delta $, where $\delta$ signifies the perturbations to the adjacency matrix of the graph. To ensure the preservation of functionality with the original malware, the subgraphs representing malicious behaviors are retained in the new graph $\hat{\mathcal{G}}$, with possibly new added nodes or edges that takes into account the characteristics of the app. When confronted with the same classifier $\mathcal{C}$ used in the malware detection task, the adversarial examples exploit the vulnerability of the neural network to yield an incorrect classification result.\\

%\jh{is it okay, to give a formulation to model the effectiveness and robustness? $ideal detection = effectiveness+robustness$, hence in the next section, we can introduce the mask mechanism and contrastive learning more naturally. For example, to achieve better effectiveness, we tailor proxy-based contrastive learning, to make the benign and malicious apps have a clear boundary. Mask mechanism can facilitate the model to learn compressed and robust representation}\\
\indent We define the power of the classifier $\mathcal{C}$ to detect malware as  \textbf{effectiveness}, and its power to detect adversarial examples as \textbf{robustness}. Current SOTA (state-of-the-art) methods have achieved impressive performance in terms of effectiveness but lack robustness in the face of adversarial examples. The typical countermeasure involves acquiring knowledge of adversarial examples, but this approach is expensive and cannot cover the entire adversarial space.
We propose that an ideal classifier should possess a holistic understanding of malicious subgraph structures to effectively counter both malware and adversarial attacks, thus achieving the goal of both effectiveness and robustness.



==> backup/3_methodology.tex <==
\section{Methodology}

\section{Methodology}
\label{sec:method}

We propose a new learning paradigm, \codename, buiding on top of the GNN framework. Specifically, we introduce a random mask mechanism to encourage the model to capture the malicious subgraph inside the input instance.
%to defend against both original malware and generated adversarial examples. 
Further more, 
%instead of using the traditional MLP as the binary classifier,
we adopt a proxy-based contrastive learning method to further compress the representations in the latent space. 
With enhanced discriminatory power, \codename is able to detect instances containing malicious information, for both original malware and adversarial examples.
We first explain the motivation of this two modules, then describe our implementations.
%\jiahao{I somehow feel Random Mask does not showcase its fancy, could we change it to anther word (Maybe Mask mechanism). the random mask is our choice, it is an implementation of our mask mechanism}
\subsection{Motivation}
\textbf{Mask Mechanism.} To encourage the model to gain a holistic understanding of the malicious behaviors represented in FCGs, we introduce a random mask into the GNN framework. Specifically, during the training phase, we randomly mask out a substantial proportion of nodes in the input FCG, forcing the remaining nodes to recover the removed representations.
From a local perspective, this strategy encourages the model to recover local patterns from partial destruction, thereby enhancing the understanding of local patterns beyond trivial statistics. Therefore, with this challenging self-supervisory task, the output representation is expected to capture the malicious structures in the form of dependencies. Since adversarial examples also retain the malicious information from their original malware instances, the learned representation is thus robust to adversarial changes in terms of the catching of malicious behaviors.\\
%\jh{Minor: flow --> what is mask mechanism, advantage, how it help android malware detection. This section is motivation, what we should emphasize is their strength and they can address the problem introduced in the last section}\\

\noindent \textbf{Proxy Based Contrastive Learning.} With a stable representation that captures the malicious information, the next step is to distinguish it from the benign representations. We adopt a proxy based contrastive loss to enhance the discrimination power of the model. The model is optimized in a way that samples within the same class cluster around their corresponding anchor, resulting in a compact region within the latent space to stabilize the classification result.


\subsection{Detector}
\label{sec:detector}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{material/framework.pdf}
    \vspace{-10pt}
    \caption{Illustration of the main framework. The training phase comprises two modules. The upper dashed-line bracket represents the self-supervised reconstruction module, while the lower bracket represent the proxy-based contrastive learning module. The detail description is shown in Section \ref{sec:detector}}
    \label{fig:framework}
    %\vspace{-10pt}
\end{figure*}
%\jiahao{Minor: Fig the hyperplane can be smaller, aligning with function call graph}

As shown in Fig \ref{fig:framework}, our model consists of two modules added upon the GNN encoder-decoder architecture : 1) a self-supervised reconstruction module, and 2) a proxy-based contrastive learning module. Specifically, in the first module, before feeding the input into the GNN encoder, we first apply a random mask to the call graph, masking out a substantial portion of the nodes in the graph. The representations, after passing through the encoder, are re-masked according to the same random mask before being fed into the decoder. The reconstruction loss encourages the model to recover the masked-out nodes from the representations of the remaining nodes, according to the dependencies that have been learned. \\
\indent In the second module, we adopt a graph readout layer to generate a graph-level representation for each instance. Then we apply the second module on the graph representations to finish the discrimination task. Specifically, we initialize
two proxy representations as the anchors of benign and malware class, respectively. During the training phase, we use cosine similarity as the metric to pull a sample closer to the anchor of its class and push it away from the anchor of a different class. The proxy representations are updated simultaneously to maintain their roles as class anchors. Prediction is made by determining which proxy the instance is closer to. \\
\indent During the testing phase, we feed the input instance through the encoder without applying the mask, and then check which proxy representation it is closer to. 


\subsection{Loss Function}
We design a self-supervised reconstruction loss to lead the learning of GNN encoder-decoder, and a supervised loss for proxy-based contrastive learning during training, respectively. For an input instance  $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{X})$, each node $v_i$ is associated its representation in the latent space $\textbf{x}_{i} \in \mathbb{R}^d$. We sample a subset of nodes $\widetilde{\mathcal{V}} \subset \mathcal{V} $ and mask their corresponding representations with a mask token [MASK], i.e., a learnable vector $\textbf{x}_{[M]} \in \mathbb{R}^d$ \cite{hou2022graphmae}. Thus, the node feature $\widetilde{\textbf{x}}_i$ for $v_i \in \mathcal{V}$ after applying the random mask can be defined as :
\[
\widetilde{\textbf{x}}_i = 
\begin{cases} 
\textbf{x}_{[M]} &   v_i \in \widetilde{\mathcal{V}}  \\
\textbf{x}_i &  v_i  \notin \widetilde{\mathcal{V}} 
\end{cases}
\]
The objective of the encoder-decoder architecture is to reconstruct the masked features of nodes in $\widetilde{\mathcal{V}}$ given the remaining features and the adjacency matrix $\mathcal{E}$. We apply uniform random sampling strategy when chosing the nodes to mask, which means that for each node, its neighbors are neither all masked nor all visible. In that case, a potential local region that represents the malicious behaviors is partially corrupted but still left with some part to recover the whole graph, encouraging the model to learn and understand its structure. After the random masking, we proceed to apply a GNN encoder $f_E$ to map each node feature $\textbf{x}_i$ from $\mathbb{R}^d$ to a more compressed latent space $\textbf{h}_i \in \mathbb{R}^h$. \\
\indent Typically in the next step, a GNN decoder $f_D$ is adopted to  maps the latent representation $\textbf{h}_i \in \mathbb{R}^h$ back to the space of the input $\mathbb{R}^d$. To further encourage the encoder to understand the underlying structures in the graphs, we proceed are-mask decoding technique before feeding  $\textbf{h}_i$ into the decoder. Specifically, the re-masked representation $\widetilde{\textbf{h}_i}$ can be denoted as follows 
\[
\widetilde{\textbf{h}}_i = 
\begin{cases} 
\textbf{h}_{[M]} &   v_i \in \widetilde{\mathcal{V}}  \\
\textbf{h}_i &  v_i  \notin \widetilde{\mathcal{V}} 
\end{cases}
\]
Then we proceed to feed $\textbf{h}_i$ into the decoder $f_D$, and force it to reconstruct the input features from the neighboring unmasked representations. The reconstructed representation is denoted as $\textbf{z}_i$. The decoder is employed only in the self-supervised learning task to assist the encoder in acquiring holistic understanding of the graph structures,  thereby aiding its success in the subsequent discrimination task. \\
\indent For the feature reconstruction criterion, we choose to leverage the cosine similarity to measure the distance between reconstructed representations and the original node representations. By employing 
$l_2$-normalization in the cosine error, vectors are mapped onto a unit hyper-sphere. This approach eliminates the impact of vector norms and improves training stability. \cite{grill2020bootstrap}. The reconstruction loss is formally defined as :
\begin{gather}
    \Lapl_{\text{rec}} = \frac{1}{|\widetilde{\mathcal{V}}|}
    \sum_{v_i\in\widetilde{\mathcal{V}}} (1 - \frac{\textbf{x}^{T}_{i}\textbf{z}_i}{\rVert \textbf{x}_i \rVert \cdot \rVert \textbf{z}_i \rVert })^{2}
\end{gather}
\indent Next, we define the proxy-based contrastive loss in the second module. With a graph readout layer, we get a graph-level representation $\textbf{g}_i$ for each graph instance, derived from the node representations given by the encoder $f_E$. Before the training start, we have already initialized two proxies for each class: $\textbf{p}_0$ for benign class and $\textbf{p}_1$ for malware class. Each instance has a supervised label $y_i$ indicating whether it belongs to benign or malware class. We formally define the contrastive loss as follows:\\
\begin{align}
    \Lapl_{\text{cl}}  
    &=   y_i \cdot
   \left[( \frac{\textbf{g}_i \cdot  \mathbf{p_0}}{\|\textbf{g}_i\| \|\mathbf{p_0}\| })^{2} +
   (1- \frac{\textbf{g}_i \cdot  \mathbf{p_1}}{\|\textbf{g}_i\| \|\mathbf{p_1}\| }  )^{2}\right] \\
   &+  (1-y_i) \cdot \left[( \frac{\textbf{g}_i\cdot  \mathbf{p_1}}{\|\textbf{g}_i\| \|\mathbf{p_1}\| })^{2} +
   (1- \frac{\textbf{g}_i \cdot  \mathbf{p_0}}{\|\textbf{g}_i\| \|\mathbf{p_0}\| }  )^{2}\right] \notag
\end{align}

Specifically, we use cosine similarity as the distance metric, pulling samples closer to the anchor of their respective classes and pushing them away from the anchor of different classes. The proxy representations are learnable vectors that are updated simultaneously during the minimization of the loss.\\
\indent Finally, with joint training, the final objective of \codename is defined as 

\begin{gather}
    \Lapl=\lambda_{1}\cdot\Lapl_{\text{rec}}+\lambda_{2}\cdot\Lapl_{\text{cl}}, 
\end{gather}
where $\lambda_1$ an $\lambda_2$ are the hyperparameters to control the strength of two modules. In the inference phase, we feed the input instance through the encoder $f_E$, proceed with a graph readout layer, then check which proxy it is closer to to determine if it is from a malicious application or not.


==> backup/5_related_work.tex <==
\section{Related Work}


==> chapters/6_discussion.tex <==
\section{Discussion}


